A Long Baseline Neutrino Oscillation Experiment Using J-PARC Neutrino Beam and Hyper-Kamiokande

Hyper-Kamiokande will be a next generation underground water Cherenkov detector with a total (fiducial) mass of 0.99 (0.56) million metric tons, approximately 20 (25) times larger than that of Super-Kamiokande. One of the main goals of Hyper-Kamiokande is the study of $CP$ asymmetry in the lepton sector using accelerator neutrino and anti-neutrino beams. In this document, the physics potential of a long baseline neutrino experiment using the Hyper-Kamiokande detector and a neutrino beam from the J-PARC proton synchrotron is presented. The analysis has been updated from the previous Letter of Intent [K. Abe et al., arXiv:1109.3262 [hep-ex]], based on the experience gained from the ongoing T2K experiment. With a total exposure of 7.5 MW $\times$ 10$^7$ sec integrated proton beam power (corresponding to $1.56\times10^{22}$ protons on target with a 30 GeV proton beam) to a $2.5$-degree off-axis neutrino beam produced by the J-PARC proton synchrotron, it is expected that the $CP$ phase $\delta_{CP}$ can be determined to better than 19 degrees for all possible values of $\delta_{CP}$, and $CP$ violation can be established with a statistical significance of more than $3\,\sigma$ ($5\,\sigma$) for $76%$ ($58%$) of the $\delta_{CP}$ parameter space.

==> ND/ND280AnalysisImprovements.tex <==
%\section{ND280 Analysis Improvements}

T2K oscillation analyses have not yet exploited the full capabilities of the near detector. While a 2.9\% uncertainty on the predicted number of electron neutrinos at the far detector has been achieved for the combination of flux and cross section parameters that are currently contained by the near detector, there remains a 7.5\% uncertainty on the far detector event sample due to additional cross section parameters that remain unconstrained.

This unconstrained uncertainty is dominated by uncertainties in the modeling of the target oxygen nucleus. Thus far, the near detector analyses have used interactions in FGD1, which is composed entirely of alternating layers of horizontally- and vertically-oriented scintillator bars. Since the FGD scintillator layers are predominantly composed of carbon and hydrogen, FGD1 measurements cannot directly probe interactions on oxygen. The downstream FGD2 contains layers of water interspersed within its scintillator layers. A simultaneous fit of the interactions in both FGDs can provide a constraint on nuclear uncertainties in oxygen, and may potentially reduce the corresponding nuclear model uncertainties. The ultimate event samples in both FGDs are shown in Table~\ref{tab:futurerates}. The statistical precision of a subtraction of interactions on scintillator from interactions on water is better than 1\%, which is more precise current detector systematic uncertainties ($\sim$3\%).

Another expected improvement to ND280 is the extension of the measured phase space of the outgoing lepton kinematics from a charged-current neutrino interaction. In the currently available analyses, muons are required to be produced in an FGD and traverse a minimum distance through the downstream TPC in order to make a measurement of both muon momentum and particle identification. This limits the muon acceptance to forward angles. Improvements to detector timing calibration and to track matching to the Electromagnetic Calorimeters (ECALs) and Side Muon Range Detectors (SMRDs) surrounding the FGDs and TPCs will allow for the reconstruction of charged-current events with backward-going and sideways-going muons. These additional samples will add less than 20\% to the total even sample, however they will be able to constrain the cross section modeling in previously inaccessible and potentially important new regions of phase space.

An additional sample of events that has not yet been incorporated into the oscillation analysis are charged-current interactions in the pi-zero detector (P0D). The P0D is capable of operating with and without water targets dispersed throughout its active volume, and by measuring the event rates separately in these two configurations, it is possible to extract constraints on interactions in water. The requirement to match a track in the TPC limits the angular acceptance for muons produced in the P0D, however the larger fiducial volume of the P0D produces a higher event sample. The expected P0D event rates are given in Table~\ref{tab:futurerates}.

\begin{table}
\begin{tabular}{|c|c|c|c|} \hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Event Sample}} & Total & Right-Sign Event \\
\multicolumn{2}{|c|}{} & Event Rate & Rate on Water \\
\multicolumn{2}{|c|}{} & (T2K, TH2K) & (T2K, T2HK) \\ \hline \hline
\multirow{4}{*}{$\nu$-mode} & FGD1 & (169,000,) & (0,0) \\
& FGD2 & (166,000,) & (84,000,)   \\
& P0D Water Out & (144,000,) & (0,0)   \\
& P0D Water In & (210,000,) & (66,000,) \\ \hline
\multirow{4}{*}{$\bar{\nu}$-mode} & FGD1 & (57,000,) & (0,0)   \\
& FGD2 & (56,000,) & (28,000,)   \\
& P0D Water Out & (63,000,) & (,)   \\
& P0D Water In & (93,000,) & (30,000,)   \\ \hline
\end{tabular}
\caption{The number of selected CC-Inclusive events in FGD1, FGD2, and the P0D are given for the ultimate expected POT assuming 50\% $\nu$-mode horn operation and 50\% $\bar{\nu}$-mode for T2K, and 30\% $\nu$-mode and 70\% $\bar{\nu}$-mode for T2HK. The subset of events that are right-sign interactions (i.e. $\nu$-interactions in $\nu$-mode and $\bar{\nu}$ interactions in $\bar{\nu}$-mode) on water are shown separately.\label{tab:futurerates}}
\end{table}

Fits to ND280 have not yet been used to constrain systematic uncertainties associated with two-body current and nucleon correlation modeling. Such a fit would require a well-motivated neutrino interaction model within which the model uncertainties are fully characterized by a set of parameters that can be constrained by the near detector data. Preliminary studies indicate that such a model would be difficult to constrain at the level required for T2HK.



==> ND/intermediate_det.tex <==
{\color{red} Description of the intermediate water cherenkov detector. (F. di Lodovico).}


==> ND/nd280_mec.tex <==
%{\color{red} Decription of the ability for ND280 to address the two body current issue (M. Hartz).}
Processes such as neutrino scattering with two-body currents or resonant production where the pion is absorbed by 
final state interactions can produce final states with no pions that do not follow quasi-elastic scattering 
kinematics.  The mismodeling of these processes can introduce biases in the relationship between neutrino 
energy and final state lepton kinematics.  Since the neutrino energy spectrum at the near and far detectors
are different due to neutrino oscillations, biases on the oscillation parameters can be introduced, even when
near detector data is used.

T2K has studied potential biases on the parameters $\theta_{23}$ and $\Delta m^{2}_{32}$ in fits to $\nu_{\mu}$
candidates at SK~\cite{Abe:2014ugx}.  Toy data for both ND280 and SK are generated using NEUT with additional 
two body current interactions based on the model of Nieves {\it et al.}~\cite{PhysRevC.83.045501}.  In addition to
the Nieves model a second ad-hoc simulation of two-body currents was studied.  This ad-hoc model was chosen to 
cover the range of two-body current calculations in the literature.
Fig.~\ref{fig:t2k_mec} illustrates the energy reconstruction
bias from two-body currents in the calculation of Nieves {\it et al.}
compared to processes that are modeled in NEUT.

\begin {figure}[htbp]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{ND/figs/mec_ebias_conf.pdf}
    \caption{The difference between the energy reconstructed assuming quasi-elastic kinematics and the true energy for 
events with no pions in the final state. Black are the NEUT simulation of CCQE events and red are the NEUT simulation of
resonant production where the $\Delta$ is absorbed.  The blue is the from the two-body current calculation of 
Nieves {\it et al.}~\cite{PhysRevC.83.045501}.}
    \label{fig:t2k_mec}
  \end{center}
\end {figure}


Both the ND280 and SK toy data are fit assuming the NEUT model,
as they are fit in the T2K oscillation analyses, and the biases on $\theta_{23}$ and $\Delta m^{2}_{32}$ are evaluated
when there are additional two-body current contributions in the toy data.  The average and RMS of the oscillation
parameter biases for many toy experiments are shown in Table.~\ref{tab:mec_bias}.  The average bias can be as large as
2.9\% on $\theta_{23}$ while there is an additional variation of the bias by as much as 3.6\%, for individual toy experiments. 
This study indicates that the modeling of two-body currents can be a dominant systematic effect, even
when ND280 data are used to constrain the neutrino interaction model.  Addressing uncertainties in the modeling of two-body
currents with additional data from the hadronic final states or novel approaches using the final state lepton kinematics will
be necessary to control these uncertainties for future experiments.

\begin{table}
\begin{center}
\caption{The oscillation parameter average bias and RMS bias of toy experiments with
two body current models. }
\label{tab:mec_bias}
\begin{tabular}{l|cc|cc}
\hline 
      & \multicolumn{2}{c|}{$\theta_{23}$} & \multicolumn{2}{c}{$\Delta m^{2}_{32}$} \\ \hline
Model & Bias Mean & Bias RMS & Bias Mean & Bias RMS   \\ \hline 
Nieves {\it et al.}~\cite{PhysRevC.83.045501}  & 0.3\%  & 3.6\% & -0.2\% & 0.6\% \\
Ad-hoc Model & -2.9\% & 3.2\% &  0.5\% &  0.6\% \\ \hline
\end{tabular}
\end{center}
\end{table}




==> ND/nd280_ultimate.tex <==
{\color{red} Discussion of the potential improvements with ND280. (M. Wilking)}

